Sample Efficient Deep Reinforcement Learning via Uncertainty Estimation

In model-free deep reinforcement learning (RL) algorithms, using noisy value estimates to supervise policy evaluation and optimization is detrimental to the sample efficiency. As this noise is heteroscedastic, its effects can be mitigated using uncertainty-based weights in the optimization process. Previous methods rely on sampled ensembles, which do not capture all aspects of uncertainty. We provide a systematic analysis of the sources of uncertainty in the noisy supervision that occurs in RL, and introduce inverse-variance RL, a Bayesian framework which combines probabilistic ensembles and Batch Inverse Variance weighting. We propose a method whereby two complementary uncertainty estimation methods account for both the Q-value and the environment stochasticity to better mitigate the negative impacts of noisy supervision. Our results show significant improvement in terms of sample efficiency on discrete and continuous control tasks.

==> biblio2.tex <==
@inproceedings{Osband_Aslanides_Cassirer_2018,
	title        = {Randomized Prior Functions for Deep Reinforcement Learning},
	author       = {Osband, Ian and Aslanides, John and Cassirer, Albin},
	year         = 2018,
	booktitle    = {Advances in Neural Information Processing Systems},
	publisher    = {Curran Associates, Inc.},
	volume       = 31,
	url          = {https://proceedings.neurips.cc/paper/2018/file/5a7b238ba0f6502e5d6be14424b20ded-Paper.pdf},
	editor       = {Bengio, S. and Wallach, H. and Larochelle, H. and Grauman, K. and Cesa-Bianchi, N. and Garnett, R.}
}
@article{ODonoghue_Osband_Munos_Mnih_2018,
	title        = {The Uncertainty Bellman Equation and Exploration},
	author       = {O’Donoghue, Brendan and Osband, Ian and Munos, Remi and Mnih, Volodymyr},
	year         = 2018,
	month        = {Oct},
	journal      = {arXiv:1709.05380},
}
@article{Dearden_Friedman_Russel_1998,
	title        = {Bayesian {Q}-Learning},
	author       = {Dearden, Richard and Friedman, Nir and Russel, Stuart J.},
	year         = 1998,
	publisher    = {AAAI},
	url          = {http://ai.stanford.edu/~nir/Papers/DFR1.pdf}
}
@article{DQN,
	title        = {Playing {Atari} with Deep Reinforcement Learning},
	author       = {Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Graves, Alex and Antonoglou, Ioannis and Wierstra, Daan and Riedmiller, Martin},
	year         = 2013,
	journal      = {NIPS},
	pages        = 9
}
@article{Mai_Khamies_Paull,
	title        = {Batch Inverse-Variance Weighting: Deep Heteroscedastic Regression},
	author       = {Mai, Vincent and Khamies, Waleed and Paull, Liam},
	year         = 2021,
	month        = {Jul},
	journal      = {arXiv:2107.04497},
}
@inproceedings{He_Init,
	title        = {Delving Deep into Rectifiers: Surpassing Human-Level Performance on {ImageNet} Classification},
	author       = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	year         = 2015,
	booktitle    = {2015 IEEE International Conference on Computer Vision (ICCV)},
	volume       = {},
	number       = {},
	pages        = {1026--1034},
	doi          = {10.1109/ICCV.2015.123}
}
 
@article{Kendall_Gal_2017, title={What Uncertainties Do We Need in Bayesian Deep Learning for Computer Vision?}, journal={arXiv:1703.04977}, author={Kendall, Alex and Gal, Yarin}, year={2017}, month={Oct} }


@article{Lakshminarayanan_Pritzel_Blundell_2017,
	title        = {Simple and Scalable Predictive Uncertainty Estimation using Deep Ensembles},
	author       = {Lakshminarayanan, Balaji and Pritzel, Alexander and Blundell, Charles},
	year         = 2017,
	month        = {Nov},
	journal      = {arXiv:1612.01474},
}
@online{Effective_sample_size_2021,
	title        = {Effective sample size},
	year         = 2021,
	month        = {Jan},
	url          = {https://en.wikipedia.org/w/index.php?title=Effective_sample_size},
	note         = {Page Version ID: 999469588},
	organization = {Wikipedia}
}
@online{Design_effects_and_effective_sample_size,
	title        = {Design Effects and Effective Sample Size},
	year         = 2017,
	month        = {Mar},
	url          = {https://docs.displayr.com/wiki/Design_Effects_and_Effective_Sample_Size},
	organization = {Displayr}
}

@article{Flennerhag_2020,
	title        = {Temporal Difference Uncertainties as a Signal for Exploration},
	author       = {Flennerhag, Sebastian and Wang, Jane X. and Sprechmann, Pablo and Visin, Francesco and Galashov, Alexandre and Kapturowski, Steven and Borsa, Diana L. and Heess, Nicolas and Barreto, Andre and Pascanu, Razvan},
	year         = 2020,
	month        = {Oct},
	journal      = {arXiv:2010.02255},
}

@article{Strens2001,
	title        = {A Bayesian Framework for Reinforcement Learning},
	author       = {Strens, Malcolm},
	year         = 2001,
	month        = {02},
	journal      = {Proceedings of the Seventeenth International Conference on Machine Learning},
	pages        = {}
}
@article{Osband_Russo_Van_Roy_2013,
	title        = {{(More)} Efficient Reinforcement Learning via Posterior Sampling},
	author       = {Osband, Ian and Russo, Daniel and Van Roy, Benjamin},
	year         = 2013,
	month        = {Jun},
	journal      = {arXiv:1306.0940v5},
}

@article{Clements_2020,
	title        = {Estimating Risk and Uncertainty in Deep Reinforcement Learning},
	author       = {Clements, William R. and Van Delft, Bastien and Robaglia, Benoît-Marie and Slaoui, Reda Bahi and Toth, Sébastien},
	year         = 2020,
	month        = {Sep},
	journal      = {arXiv:1905.09638},
}
@article{Lee_Laskin_Srinivas_Abbeel_2020,
	title        = {{SUNRISE}: A Simple Unified Framework for Ensemble Learning in Deep Reinforcement Learning},
	author       = {Lee, Kimin and Laskin, Michael and Srinivas, Aravind and Abbeel, Pieter},
	year         = 2020,
	month        = {Jul},
	journal      = {arXiv:2007.04938},
}
@article{Osband_Roy_Russo_Wen_2019,
	title        = {Deep Exploration via Randomized Value Functions},
	author       = {Osband, Ian and Roy, Benjamin Van and Russo, Daniel J. and Wen, Zheng},
	year         = 2019,
	journal      = {Journal of Machine Learning Research},
	volume       = 20,
	number       = 124,
	pages        = {1–62}
}
@article{Osband_Blundell_Pritzel_Van_Roy_2016,
	title        = {Deep Exploration via Bootstrapped {DQN}},
	author       = {Osband, Ian and Blundell, Charles and Pritzel, Alexander and Van Roy, Benjamin},
	year         = 2016,
	month        = {Jul},
	journal      = {arXiv:1602.04621 },
}

@article{Thompson_1933,
	title        = {On the Likelihood that One Unknown Probability Exceeds Another in View of the Evidence of Two Samples},
	author       = {Thompson, William R.},
	year         = 1933,
	month        = {Dec},
	journal      = {Biometrika},
	volume       = 25,
	number       = {3/4},
	pages        = 285,
	doi          = {10.2307/2332286},
	issn         = {00063444}
}
@article{Aravindan_Lee_2021,
	title        = {State-Aware Variational Thompson Sampling for Deep {Q}-Networks},
	author       = {Aravindan, Siddharth and Lee, Wee Sun},
	year         = 2021,
	month        = {Feb},
	journal      = {arXiv:2102.03719},
}
@article{Fortunato_2019,
	title        = {Noisy Networks for Exploration},
	author       = {Fortunato, Meire and Azar, Mohammad Gheshlaghi and Piot, Bilal and Menick, Jacob and Osband, Ian and Graves, Alex and Mnih, Vlad and Munos, Remi and Hassabis, Demis and Pietquin, Olivier and et al.},
	year         = 2019,
	month        = {Jul},
	journal      = {arXiv:1706.10295},
}
@article{Jain_Lahlou_2021,
	title        = {{DEUP}: Direct Epistemic Uncertainty Prediction},
	author       = {Jain, Moksh and Lahlou, Salem and Nekoei, Hadi and Butoi, Victor and Bertin, Paul and Rector-Brooks, Jarrid and Korablyov, Maksym and Bengio, Yoshua},
	year         = 2021,
	month        = {Feb},
	journal      = {arXiv:2102.08501},
}

@article{Pathak_Agrawal_Efros_Darrell_2017,
	title        = {Curiosity-driven Exploration by Self-supervised Prediction},
	author       = {Pathak, Deepak and Agrawal, Pulkit and Efros, Alexei A. and Darrell, Trevor},
	year         = 2017,
	month        = {May},
	journal      = {arXiv:1705.05363},
}

@article{Buckman_Hafner_Tucker_Brevdo_Lee_2019,
	title        = {Sample-Efficient Reinforcement Learning with Stochastic Ensemble Value Expansion},
	author       = {Buckman, Jacob and Hafner, Danijar and Tucker, George and Brevdo, Eugene and Lee, Honglak},
	year         = 2019,
	month        = {Jun},
	journal      = {arXiv:1807.01675},
}

@inproceedings{gal2016improving,
	title        = {Improving {PILCO} with Bayesian neural network dynamics models},
	author       = {Gal, Yarin and McAllister, Rowan and Rasmussen, Carl Edward},
	year         = 2016,
	booktitle    = {Data-Efficient Machine Learning workshop, ICML},
	volume       = 4,
	number       = 34,
	pages        = 25
}
@article{Depeweg_2017,
	title        = {Learning and Policy Search in Stochastic Dynamical Systems with Bayesian Neural Networks},
	author       = {Depeweg, Stefan and Hernández-Lobato, José Miguel and Doshi-Velez, Finale and Udluft, Steffen},
	year         = 2017,
	month        = {Mar},
	journal      = {arXiv:1605.07127},
}

@article{Chua_Calandra_McAllister_Levine_2018,
	title        = {Deep Reinforcement Learning in a Handful of Trials using Probabilistic Dynamics Models},
	author       = {Chua, Kurtland and Calandra, Roberto and McAllister, Rowan and Levine, Sergey},
	year         = 2018,
	month        = {Nov},
	journal      = {arXiv:1805.12114},
}

@article{Kahn_Villaflor_Pong_Abbeel_Levine_2017,
	title        = {Uncertainty-Aware Reinforcement Learning for Collision Avoidance},
	author       = {Kahn, Gregory and Villaflor, Adam and Pong, Vitchyr and Abbeel, Pieter and Levine, Sergey},
	year         = 2017,
	month        = {Feb},
	journal      = {arXiv:1702.01182},
}

@inproceedings{Lutjens_2019,
	title        = {Safe Reinforcement Learning With Model Uncertainty Estimates},
	author       = {Lütjens, Björn and Everett, Michael and How, Jonathan P.},
	year         = 2019,
	booktitle    = {2019 International Conference on Robotics and Automation (ICRA)},
	volume       = {},
	number       = {},
	pages        = {8662--8668},
	doi          = {10.1109/ICRA.2019.8793611}
}
@inproceedings{gal16,
	title        = {Dropout as a Bayesian Approximation: Representing Model Uncertainty in Deep Learning},
	author       = {Gal, Yarin and Ghahramani, Zoubin},
	year         = 2016,
	month        = {20--22 Jun},
	booktitle    = {Proceedings of The 33rd International Conference on Machine Learning},
	publisher    = {PMLR},
	address      = {New York, New York, USA},
	series       = {Proceedings of Machine Learning Research},
	volume       = 48,
	pages        = {1050--1059},
	editor       = {Balcan, Maria Florina and Weinberger, Kilian Q.},
	pdf          = {http://proceedings.mlr.press/v48/gal16.pdf}
}
@article{Wen_Tran_Ba_2020,
	title        = {{BatchEnsemble}: An Alternative Approach to Efficient Ensemble and Lifelong Learning},
	author       = {Wen, Yeming and Tran, Dustin and Ba, Jimmy},
	year         = 2020,
	month        = {Feb},
	journal      = {arXiv:2002.06715v2},
}

@article{Dusenberry_Jerfel_Wen_Ma_Snoek_Heller_Lakshminarayanan_Tran_2020,
	title        = {Efficient and Scalable Bayesian Neural Nets with Rank-1 Factors},
	author       = {Dusenberry, Michael W. and Jerfel, Ghassen and Wen, Yeming and Ma, Yi-an and Snoek, Jasper and Heller, Katherine and Lakshminarayanan, Balaji and Tran, Dustin},
	year         = 2020,
	month        = {May},
	journal      = {arXiv:2005.07186v1},
}

@article{Franchi_Bursuc_Aldea_Dubuisson_Bloch_2020,
	title        = {Encoding the latent posterior of Bayesian Neural Networks for uncertainty quantification},
	author       = {Franchi, Gianni and Bursuc, Andrei and Aldea, Emanuel and Dubuisson, Severine and Bloch, Isabelle},
	year         = 2020,
	month        = {Dec},
	journal      = {arXiv:2012.02818v2},
}

@article{Mobiny_Nguyen_Moulik_Garg_Wu_2019,
	title        = {DropConnect Is Effective in Modeling Uncertainty of Bayesian Deep Networks},
	author       = {Mobiny, Aryan and Nguyen, Hien V. and Moulik, Supratik and Garg, Naveen and Wu, Carol C.},
	year         = 2019,
	month        = {Jun},
	journal      = {arXiv:1906.04569v1},
}

@article{MacKay_1992,
	title        = {A Practical Bayesian Framework for Backpropagation Networks},
	author       = {MacKay, David J. C.},
	year         = 1992,
	month        = {May},
	journal      = {Neural Computation},
	volume       = 4,
	number       = 3,
	pages        = {448–472},
	doi          = {10.1162/neco.1992.4.3.448},
	issn         = {0899-7667, 1530-888X}
}
@article{Ovadia_2019,
	title        = {Can You Trust Your Model’s Uncertainty? {Evaluating} Predictive Uncertainty Under Dataset Shift},
	author       = {Ovadia, Yaniv and Fertig, Emily and Ren, Jie and Nado, Zachary and Sculley, D. and Nowozin, Sebastian and Dillon, Joshua V. and Lakshminarayanan, Balaji and Snoek, Jasper},
	year         = 2019,
	month        = {Dec},
	journal      = {arXiv:1906.02530},
}

@article{Kumar_Gupta_Levine_2020,
	title        = {{DisCor}: Corrective Feedback in Reinforcement Learning via Distribution Correction},
	author       = {Kumar, Aviral and Gupta, Abhishek and Levine, Sergey},
	year         = 2020,
	month        = {Mar},
	journal      = {arXiv:2003.07305},
}
@article{Kumar_Fu_Tucker_Levine_2019,
	title        = {Stabilizing Off-Policy {Q}-Learning via Bootstrapping Error Reduction},
	author       = {Kumar, Aviral and Fu, Justin and Tucker, George and Levine, Sergey},
	year         = 2019,
	month        = {Nov},
	journal      = {arXiv:1906.00949},
}

@article{OpenAIGym,
	title        = {{OpenAI Gym}},
	author       = {Brockman, Greg and Cheung, Vicki and Pettersson, Ludwig and Schneider, Jonas and Schulman, John and Tang, Jie and Zaremba, Wojciech},
	year         = 2016,
	month        = {Jun},
	journal      = {arXiv:1606.01540},
}

@article{Haarnoja_Zhou_Abbeel_Levine_2018,
	title        = {Soft Actor-Critic: Off-Policy Maximum Entropy Deep Reinforcement Learning with a Stochastic Actor},
	author       = {Haarnoja, Tuomas and Zhou, Aurick and Abbeel, Pieter and Levine, Sergey},
	year         = 2018,
	journal      = {arXiv:1801.01290},
}

@article{Schulman_Wolski_Dhariwal_Radford_Klimov_2017,
	title        = {Proximal Policy Optimization Algorithms},
	author       = {Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg},
	year         = 2017,
	month        = {Aug},
	journal      = {arXiv:1707.06347},
}
@inbook{Brandt_2014,
	title        = {Linear and Polynomial Regression},
	author       = {Brandt, Siegmund},
	year         = 2014,
	booktitle    = {Data Analysis: Statistical and Computational Methods for Scientists and Engineers},
	publisher    = {Springer International Publishing},
	pages        = {321–329},
	doi          = {10.1007/978-3-319-03762-2_12},
	isbn         = {978-3-319-03762-2},
	place        = {Cham}
}

@book{Bishop_2006,
	title        = {Pattern recognition and machine learning},
	author       = {Bishop, Christopher M.},
	year         = 2006,
	publisher    = {Springer},
	series       = {Information science and statistics},
	isbn         = {978-0-387-31073-2},
	place        = {New York},
	collection   = {Information science and statistics}
}

@book{Siegwart_Nourbakhsh_Scaramuzza_2011,
	title        = {Introduction to Autonomous Mobile Robots},
	author       = {Siegwart, R. and Nourbakhsh, I.R. and Scaramuzza, D.},
	year         = 2011,
	publisher    = {MIT Press},
	series       = {Intelligent Robotics and Autonomous Agents series},
	isbn         = {978-0-262-01535-6},
	collection   = {Intelligent Robotics and Autonomous Agents series}
}

@book{Sutton_Barto_2018,
	title        = {Reinforcement learning: an introduction},
	author       = {Sutton, Richard S. and Barto, Andrew G.},
	year         = 2018,
	publisher    = {The MIT Press},
	series       = {Adaptive computation and machine learning series},
	isbn         = {978-0-262-03924-6},
	place        = {Cambridge, Massachusetts},
	edition      = {Second edition},
	collection   = {Adaptive computation and machine learning series}
}

@article{OpenAI_Five_Dota,
	title        = {Dota 2 with Large Scale Deep Reinforcement Learning},
	author       = {{OpenAI} and Berner, Christopher and Brockman, Greg and Chan, Brooke and Cheung, Vicki and Debiak, Przemyslaw and Dennison, Christy and Farhi, David and Fischer, Quirin and Hashme, Shariq and et al.},
	year         = 2019,
	month        = {Dec},
	journal      = {arXiv:1912.06680},
}
@article{AlphaGo,
	title        = {Mastering the game of {Go} with deep neural networks and tree search},
	author       = {Silver, David and Huang, Aja and Maddison, Chris J. and Guez, Arthur and Sifre, Laurent and van den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and et al.},
	year         = 2016,
	month        = {Jan},
	journal      = {Nature},
	volume       = 529,
	number       = 7587,
	pages        = {484–489},
	doi          = {10.1038/nature16961},
	issn         = {0028-0836, 1476-4687}
}
@article{Wu_Zhai_Srivastava_Susskind_Zhang_Salakhutdinov_Goh_2021,
	title        = {Uncertainty Weighted Actor-Critic for Offline Reinforcement Learning},
	author       = {Wu, Yue and Zhai, Shuangfei and Srivastava, Nitish and Susskind, Joshua and Zhang, Jian and Salakhutdinov, Ruslan and Goh, Hanlin},
	year         = 2021,
	month        = {May},
	journal      = {arXiv:2105.08140},
}

@article{PPO, 
    title       = {Proximal Policy Optimization Algorithms}, 
    ISSN        = {0008-5286 (Print)r0008-5286 (Linking)}, 
    DOI         = {10.1007/s00038-010-0125-8}, 
    author      = {Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg}, 
    year        = {2017}, 
    pages       = {1–12}
}
@inproceedings{Nix_Weigend_1994,
	title        = {Estimating the mean and variance of the target probability distribution},
	author       = {Nix, D.A. and Weigend, A.S.},
	year         = 1994,
	booktitle    = {Proceedings of 1994 IEEE International Conference on Neural Networks (ICNN’94)},
	publisher    = {IEEE},
	pages        = {55–60 vol.1},
	doi          = {10.1109/ICNN.1994.374138},
	isbn         = {978-0-7803-1901-1},
	place        = {Orlando, FL, USA}
}
@article{Chen_Sidor_Abbeel_Schulman_2017,
	title        = {{UCB} Exploration via {Q}-Ensembles},
	author       = {Chen, Richard Y. and Sidor, Szymon and Abbeel, Pieter and Schulman, John},
	year         = 2017,
	month        = {Nov},
	journal      = {arXiv:1706.01502},
}
@article{DDPG,
	title        = {Continuous control with deep reinforcement learning},
	author       = {Lillicrap, Timothy P. and Hunt, Jonathan J. and Pritzel, Alexander and Heess, Nicolas and Erez, Tom and Tassa, Yuval and Silver, David and Wierstra, Daan},
	year         = 2019,
	month        = {Jul},
	journal      = {arXiv:1509.02971},
}
@article{TD3,
	title        = {Addressing Function Approximation Error in Actor-Critic Methods},
	author       = {Fujimoto, Scott and van Hoof, Herke and Meger, David},
	year         = 2018,
	month        = {Oct},
	journal      = {arXiv:1802.09477},
}
@book{Murphy_2012,
	title        = {Machine learning: a probabilistic perspective},
	author       = {Murphy, Kevin P.},
	year         = 2012,
	publisher    = {MIT Press},
	series       = {Adaptive computation and machine learning series},
	isbn         = {978-0-262-01802-9},
	place        = {Cambridge, MA},
	collection   = {Adaptive computation and machine learning series}
}
@article{Henderson_Islam_Bachman_Pineau_Precup_Meger_2019,
	title        = {Deep Reinforcement Learning that Matters},
	author       = {Henderson, Peter and Islam, Riashat and Bachman, Philip and Pineau, Joelle and Precup, Doina and Meger, David},
	year         = 2019,
	month        = {Jan},
	journal      = {arXiv:1709.06560},
}
@article{Levi_Gispan_Giladi_Fetaya_2020,
	title        = {Evaluating and Calibrating Uncertainty Prediction in Regression Tasks},
	author       = {Levi, Dan and Gispan, Liran and Giladi, Niv and Fetaya, Ethan},
	year         = 2020,
	month        = {Feb},
	journal      = {arXiv:1905.11659},
}
@article{Kuleshov_Fenner_Ermon_2018,
	title        = {Accurate Uncertainties for Deep Learning Using Calibrated Regression},
	author       = {Kuleshov, Volodymyr and Fenner, Nathan and Ermon, Stefano},
	year         = 2018,
	month        = {Jun},
	journal      = {arXiv:1807.00263},
}
@article{bsuite,
	title        = {Behaviour Suite for Reinforcement Learning},
	author       = {Osband, Ian and Doron, Yotam and Hessel, Matteo and Aslanides, John and Sezener, Eren and Saraiva, Andre and McKinney, Katrina and Lattimore, Tor and Szepesvari, Csaba and Singh, Satinder and et al.},
	year         = 2020,
	month        = {Feb},
	journal      = {arXiv:1908.03568},
}
@article{MBBL,
	title        = {Benchmarking Model-Based Reinforcement Learning},
	author       = {Wang, Tingwu and Bao, Xuchan and Clavera, Ignasi and Hoang, Jerrick and Wen, Yeming and Langlois, Eric and Zhang, Shunshi and Zhang, Guodong and Abbeel, Pieter and Ba, Jimmy},
	year         = 2019,
	month        = {Jul},
	journal      = {arXiv:1907.02057},
}
@article{Bhatt_Mani_Bansal_Murthy_Lee_Paull_2021,
	title        = {$f$-{Cal}: Calibrated aleatoric uncertainty estimation from neural networks for robot perception},
	author       = {Bhatt, Dhaivat and Mani, Kaustubh and Bansal, Dishank and Murthy, Krishna and Lee, Hanju and Paull, Liam},
	year         = 2021,
	month        = {Sep},
	journal      = {arXiv:2109.13913},
}
@misc{universite2018montreal,
	title        = {Montreal Declaration for a Responsible Development of Artificial Intelligence},
	author       = {{Université de Montréal}},
	year         = 2018,
	publisher    = {Universite de Montreal}
}
@article{lacoste2019quantifying,
	title        = {Quantifying the Carbon Emissions of Machine Learning},
	author       = {Lacoste, Alexandre and Luccioni, Alexandra and Schmidt, Victor and Dandres, Thomas},
	year         = 2019,
	journal      = {arXiv:1910.09700}
}
@article{Bellemare_Dabney_Munos_2017,
	title        = {A Distributional Perspective on Reinforcement Learning},
	author       = {Bellemare, Marc G. and Dabney, Will and Munos, Rémi},
	year         = 2017,
	month        = {Jul},
	journal      = {arXiv:1707.06887},
}
@article{Hullermeier_Waegeman_2021,
	title        = {Aleatoric and epistemic uncertainty in machine learning: an introduction to concepts and methods},
	author       = {Hüllermeier, Eyke and Waegeman, Willem},
	year         = 2021,
	month        = {Mar},
	journal      = {Machine Learning},
	volume       = 110,
	number       = 3,
	pages        = {457–506},
	doi          = {10.1007/s10994-021-05946-3},
	issn         = {0885-6125, 1573-0565}
}
@report{delayedRewards,
	title        = {Handling stochastic reward delays in machine reinforcement learning},
	author       = {Campbell, J.S. (Jeffrey S.) and Givigi, S.N. (Sidney N.) and Schwartz, Howard M.},
	year         = 2015,
	month        = jan,
	booktitle    = {Canadian Conference on Electrical and Computer Engineering},
	pages        = {314--319},
	doi          = {10.1109/CCECE.2015.7129295}
}
@article{Romoff2018,
	title        = {Reward Estimation for Variance Reduction in Deep Reinforcement Learning},
	author       = {Romoff, Joshua and Henderson, Peter and Piché, Alexandre and François-Lavet, Vincent and Pineau, Joelle},
	year         = 2018,
	number       = {CoRL},
	pages        = {1–26}
}

@article{NelderMead,
    author = {Nelder, J. A. and Mead, R.},
    title = "{A Simplex Method for Function Minimization}",
    journal = {The Computer Journal},
    volume = {7},
    number = {4},
    pages = {308-313},
    year = {1965},
    month = {01},
    issn = {0010-4620},
    doi = {10.1093/comjnl/7.4.308},
    eprint = {https://academic.oup.com/comjnl/article-pdf/7/4/308/1013182/7-4-308.pdf},
}

 @article{Kothari_Perone_Bergamini_Alahi_Ondruska_2021, title={DriverGym: Democratising Reinforcement Learning for Autonomous Driving},  journal={arXiv:2111.06889 }, author={Kothari, Parth and Perone, Christian and Bergamini, Luca and Alahi, Alexandre and Ondruska, Peter}, year={2021}, month={Nov} }

 @article{Sunderhauf_2018, title={The limits and potentials of deep learning for robotics}, volume={37}, ISSN={0278-3649}, DOI={10.1177/0278364918770733},  number={4–5}, journal={The International Journal of Robotics Research}, publisher={SAGE Publications Ltd STM}, author={Sünderhauf, Niko and Brock, Oliver and Scheirer, Walter and Hadsell, Raia and Fox, Dieter and Leitner, Jürgen and Upcroft, Ben and Abbeel, Pieter and Burgard, Wolfram and Milford, Michael and et al.}, year={2018}, month={Apr}, pages={405–420} }

 @article{Kingma_Ba_2017, title={Adam: A Method for Stochastic Optimization}, url={http://arxiv.org/abs/1412.6980}, note={arXiv: 1412.6980}, journal={arXiv:1412.6980 [cs]}, author={Kingma, Diederik P. and Ba, Jimmy}, year={2017}, month={Jan} }
 
  @article{Dulac_2019, title={Challenges of Real-World Reinforcement Learning}, journal={arXiv:1904.12901}, author={Dulac-Arnold, Gabriel and Mankowitz, Daniel and Hester, Todd}, year={2019}, month={Apr} }

 @article{Liu_Nageotte_Zanne_deMathelin_DrespLangley_2021, title={Deep Reinforcement Learning for the Control of Robotic Manipulation: A Focussed Mini-Review}, volume={10}, ISSN={2218-6581}, DOI={10.3390/robotics10010022},  note={arXiv: 2102.04148}, number={1}, journal={Robotics}, author={Liu, Rongrong and Nageotte, Florent and Zanne, Philippe and de Mathelin, Michel and Dresp-Langley, Birgitta}, year={2021}, month={Jan}, pages={22} }

